DanceTrack: Multi-Object Tracking in Uniform Appearance and Diverse Motion

A typical pipeline for multi-object tracking (MOT) is to use a detector for object localization, and following re-identification (re-ID) for object association. This pipeline is partially motivated by recent progress in both object detection and re-ID, and partially motivated by biases in existing tracking datasets, where most objects tend to have distinguishing appearance and re-ID models are sufficient for establishing associations. In response to such bias, we would like to re-emphasize that methods for multi-object tracking should also work when object appearance is not sufficiently discriminative. To this end, we propose a large-scale dataset for multi-human tracking, where humans have similar appearance, diverse motion and extreme articulation. As the dataset contains mostly group dancing videos, we name it "DanceTrack". We expect DanceTrack to provide a better platform to develop more MOT algorithms that rely less on visual discrimination and depend more on motion analysis. We benchmark several state-of-the-art trackers on our dataset and observe a significant performance drop on DanceTrack when compared against existing benchmarks. The dataset, project code and competition server are released at: \url{https://github.com/DanceTrack}.

==> tables/table_data.tex <==
\setlength{\tabcolsep}{4.5mm}
\begin{tabular}{l c | l l l l l}
\toprule
Data & Ass. & HOTA & DetA & AssA & MOTA & IDF1  \\
\midrule
DanceTrack & box & 36.9 & 63.6 & 21.6 & 78.8 & 39.2\\
+ COCObox~\cite{COCO} & box & 
38.1 \textcolor{codegreen}{(+\textbf{1.2})}  & 
64.3 \textcolor{codegreen}{(+\textbf{0.7})} 	& 
22.7 \textcolor{codegreen}{(+\textbf{1.1})} 	& 
80.8 \textcolor{codegreen}{(+\textbf{2.0})} & 
40.4 \textcolor{codegreen}{(+\textbf{1.2})} \\
\bottomrule
\end{tabular}

==> tables/table_data_stat.tex <==
\setlength{\tabcolsep}{1.0mm}
\begin{tabular}{l | c | c }
\toprule
Dataset &  Adjacent IoU & Rel-Pos Switch\\
\midrule
MOT17~\cite{MOT16} &  0.9395849987555913 & 0.0011418627159023229 \\
MOT20~\cite{MOT20} & 0.959701854053389 & 0.0075975684532390165 \\
% WILDTRACK & \\
KITTI~\cite{KITTI} &0.7910263022999612 & 0.013729313797828607 \\
KITTI-pedestrian &0.7731744307330137 & 0.01661983619298140 \\
BDD100K~\cite{BDD} & 0.6366456529833184 & 0.029016356054376507 \\
BDD100K-pedestrian & 0.6611333761677615 & 0.024788481448019945 \\ 
% Waymo~\cite{waymo} & \\
DanceTrack & 0.8929760750716758 & 0.02161598955987687\\
DanceTrack-hard & 0.8900754088811057 & 0.03794712984156905\\
\bottomrule
\end{tabular}

==> tables/table_ddd.tex <==
\setlength{\tabcolsep}{4.2mm}
\begin{tabular}{l c |l l l l l}
\toprule
Data & Ass. & HOTA & DetA & AssA & MOTA & IDF1  \\
\midrule
DanceTrack & box & 36.9 & 63.6 & 21.6 & 78.8 & 39.2\\
+ KITTI & box & 34.4 \downscore{2.5} & 57.8	\downscore{5.8} & 20.7 \downscore{0.9} & 72.9 \downscore{5.9} & 38.5 \downscore{0.7} \\ 
+ KITTI & + depth  & 
35.1 \textcolor{codegreen}{(+\textbf{0.7})} & 
57.3 \downscore{0.5}& 
21.6 \textcolor{codegreen}{(+\textbf{0.9})} & 
72.8 \downscore{0.1}& 
40.2 \textcolor{codegreen}{(+\textbf{1.7})} \\

				
\bottomrule
\end{tabular}

==> tables/table_mask.tex <==
\setlength{\tabcolsep}{4.2mm}
\begin{tabular}{l c |l l l l l}
\toprule
Data & Ass. & HOTA & DetA & AssA & MOTA & IDF1  \\
\midrule
DanceTrack & box & 36.9 & 63.6 & 21.6 & 78.8 & 39.2\\
+ COCOmask~\cite{COCO} & box & 38.1	\upscore{1.2} & 64.5 \upscore{0.9} & 22.6  \upscore{1.0} & 80.6 \upscore{1.8} & 40.3 \upscore{1.1} \\ 
+ COCOmask & + mask & 39.2 \upscore{1.1} & 
64.9 \upscore{0.4}	& 
23.9 \textcolor{codegreen}{(+\textbf{1.3})}& 
80.7 \upscore{0.1} & 
41.6 \textcolor{codegreen}{(+\textbf{0.3})}\\

\bottomrule
\end{tabular}

==> tables/table_pose.tex <==
\setlength{\tabcolsep}{4.2mm}
\begin{tabular}{l c | l l l l l}
\toprule
Data & Ass. & HOTA & DetA & AssA & MOTA & IDF1  \\
\midrule
DanceTrack & box & 36.9 & 63.6 & 21.6 & 78.8 & 39.2\\
+ COCOpose & box & 40.6 \upscore{3.7} & 65.5 \upscore{1.9} & 25.3 \upscore{3.7} & 82.9 \upscore{4.1} & 42.9 \upscore{3.7}\\ 
+ COCOpose & + pose & 
41.0 \upscore{0.4} & 
65.9 \upscore{0.4} & 
25.6 \upscore{0.3} & 
83.1 \upscore{0.3} &
43.9 \textcolor{codegreen}{(+\textbf{1.0})} \\

\bottomrule
\end{tabular}
